Optimism and Delays in Episodic Reinforcement Learning

There are many algorithms for regret minimisation in episodic reinforcement learning. This problem is well-understood from a theoretical perspective, providing that the sequences of states, actions and rewards associated with each episode are available to the algorithm updating the policy immediately after every interaction with the environment. However, feedback is almost always delayed in practice. In this paper, we study the impact of delayed feedback in episodic reinforcement learning from a theoretical perspective and propose two general-purpose approaches to handling the delays. The first involves updating as soon as new information becomes available, whereas the second waits before using newly observed information to update the policy. For the class of optimistic algorithms and either approach, we show that the regret increases by an additive term involving the number of states, actions, episode length, the expected delay and an algorithm-dependent constant. We empirically investigate the impact of various delay distributions on the regret of optimistic algorithms to validate our theoretical results.

==> figures/agent-environment.tex <==
% Standard Diagram
% ----------------
% \begin{figure}[h]
%     \centering
%     \begin{tikzpicture}[node distance=1cm, auto,]
%     \node[] (agent) {Agent ($\pi_{k}$)};
%     \node[inner sep = 5pt, below=2cm of agent] (reward) {$r_{h} \sim R_{h}(s_{h}, a_{h})$};
%     \node[inner sep = 5pt, right=3cm of reward] (action) {$a_h \sim \pi_{k}\,(s_{h}, h)$};
%     \node[inner sep = 5pt, left=3cm of reward] (state) {$s_{h + 1} \sim P_{h}\,(\cdot\vert s_{h}, a_{h})$};
%     \node[inner sep=5pt, below=2cm of reward] (env) {Environment};

    
    
%     \draw[thick, shorten <=2pt, shorten >=2pt, above](env.north)-|(reward);
%     \draw[-{Latex[length=.375cm]}, thick, shorten <=2pt, shorten >=2pt, above](reward.north)-|(agent.south);
    
%     \draw[thick, shorten <=2pt, shorten >=2pt, rounded corners=5pt] (agent)-|(action);
%     \draw[-{Latex[length=.375cm]}, thick, shorten <=2pt, shorten >=2pt, rounded corners=5pt] (action)|-(env);
    
%     \draw[thick, shorten <=2pt, shorten >=2pt,rounded corners=5pt] (env)-|(state);
%     \draw[-{Latex[length=.375cm]}, thick, shorten <=2pt, shorten >=2pt, rounded corners=5pt] (state)|-(agent);
%     \end{tikzpicture}
%     \caption{Visual representation of the agent-environment interaction.}
%     \label{fig: agent-environment interaction}
% \end{figure}

% Layout 1
% --------
\begin{figure}
\centering
\begin{tikzpicture}[
auto,
    block/.style={
      rectangle,
      draw=black,
      thick,
     text width=5.75em,
      rounded corners,
      minimum height=2.5em,
      text centered
    },
    line/.style={
      draw,thick,
      -latex',
      shorten >=2pt
    },
    cloud/.style={
      draw=red,
      thick,
      ellipse,
      fill=red!20,
      minimum height=1em
    }
  ]
]
    \node[block] (Base) {Base};
    \node[below = 3cm of Base] (Center) {};
    \node[block, below = 6cm of Base](Environment) {Environment};
    \node[right = 7cm of Environment](Policy){$\pi_{k}$};
    \node[left = 7cm of Environment](Buffer){Buffer};
    \node[above = 2cm of Buffer, text centered] (Feedback) {$\{\mathcal{D}_{i}: i + \tau_{i} < k + 1\}$};
    \node[below = 2cm of Buffer](Data){$\mathcal{D}_{k}$};
    \node[block, below = 4cm of Environment](Agent){Agent$(\pi_{k})$};

    % draw arrows around the diagram
    \draw[thick, shorten <=2pt, shorten >=2pt, rounded corners=50pt] (Base)-|(Policy);
    \draw[-{Latex[length=.5cm]}, thick, shorten <=2pt, shorten >=2pt, rounded corners=50pt] (Policy)|-(Agent);

    \draw[thick, shorten <=2pt, shorten >=2pt, rounded corners=50pt] (Agent)-|(Data);
    \draw[-{Latex[length=.5cm]}, thick, shorten <=2pt, shorten >=2pt] (Data)--(Buffer);

    \draw[thick, shorten <=2pt, shorten >=2pt] (Buffer)--(Feedback);
    \draw[-{Latex[length=.5cm]}, thick, shorten <=2pt, shorten >=2pt, rounded corners=50pt] (Feedback.north)|-(Base);
    
    % draw box around the agent-environment interaction
    \draw[black, very thick, rounded corners] ($(Environment.north west)+(-2,1)$)  rectangle ($(Agent.south east)+(2,-1)$);
    \draw[-{Latex[length=.5cm]}, thick, shorten <=10pt, shorten >=10pt] (Agent.110) to[bend left = 45] (Environment.250);
    \draw[-{Latex[length=.5cm]}, thick, shorten <=10pt, shorten >=10pt] (Environment.290) to[bend left = 45] (Agent.70);
    
    % % agent-environment interaction arrows
    % \draw[-{Latex[length=.5cm]}, thick] (Agent.120)-|(Environment.240);
    % \draw[-{Latex[length=.5cm]}, thick] (Environment.300)-|(Agent.60);

    
\end{tikzpicture}
\caption{Visual representation of the agent-environment interaction.}
\label{fig: agent-environment interaction}
\end{figure}
% Layout 4
% --------
% \begin{figure}[h]
% \begin{tikzpicture}[node distance=1cm, auto,]
%     \centering
%     % draw vertical lines
%     \foreach \x in {0, 5, 10, 15, 20}
%     \draw (\x cm,12pt) -- (\x cm,-12pt);

%     % label the vertical lines
%     \foreach \x/\descr in {0/1, 5/2, 10/3, 15/4, 20/5}
%     \node[] at (\x,-30pt) {$\descr$};

%     \node[rectangle, draw, minimum width=25cm, minimum height = 2cm] at (12.5, 65pt){Base};

%     % draw the arrow going through vertical lines
%     \draw[-{Latex[length=.5cm]}] (0, 0)--(25, 0);

%     \node[align = right] at (-110pt, -30pt) {Episode};
%     \node[align = right] at (-110pt, -80pt) {Feedback};
%     %\node[align = right] at (-110pt, -80pt) {Policy};
%     %\node[align = right] at (-110pt, -130pt) {Feedback};
    
%     % add policies 
%     \foreach \x/\descr in {0/$\pi_1$, 5/$\pi_2$, 10/$\pi_3$, 15/$\pi_4$, 20/$\pi_5$}
%     \node[] at (\x, 170pt) {\descr};

%     \draw[black] (0, 100pt) to node [below = 0pt]{} (0, 150pt);
%     \draw[black] (5, 100pt) to node [below = 0pt]{} (5, 150pt) ;
%     \draw[black] (10, 100pt) to node [below = 0pt]{} (10, 150pt) ;
%     \draw[black] (15, 100pt) to node [below = 0pt]{} (15, 150pt) ;
%     \draw[black] (20, 100pt) to node [below = 0pt]{} (20, 150pt) ;

%     %% label the vertical lines
%     % \foreach \x/\descr in {0/$\pi_1$, 5/$\pi_2$, 10/$\pi_3$, 15/$\pi_4$, 20/$\pi_5$}
%     % \node[] at (\x,-80pt) {\descr};

%     % label the vertical lines
%     \foreach \x/\descr in {0/$\emptyset$, 5/$\emptyset$, 10/$\mathcal{D}_1$, 15/$\mathcal{D}_3$, 20/$\mathcal{D}_2$}
%     % \node[] at (\x,-130pt) {\descr};
%     \node[] at (\x,-80pt) {\descr};
    
%     % draw the delays on to the timeline
%     \draw[red, -{Latex[length=.5cm]}] (0, -105pt) to [bend right=50] node [below = .25cm]{$\tau_{1}$} (10 - 0.05, -105pt) ;
%     \draw[red, -{Latex[length=.5cm]}] (5, -105pt) to [bend right=50] node [below = .25cm]{$\tau_{2}$} (20 - 0.05, -105pt) ;
%     \draw[red, -{Latex[length=.5cm]}] (10, -105pt) to [bend right=50] node [below = .25cm]{$\tau_{3}$} (15 - 0.05, -105pt) ;
%     \draw[red, -{Latex[length=.5cm]}] (15, -105pt) to [bend right=50] node [below = .25cm]{$\tau_{4}$} (25 - 0.05, -135pt) ;
% \end{tikzpicture}
% \label{fig: base-environment interaction}
% \caption{Illustration of delayed feedback.}
% \end{figure}

==> figures/experiment-diagram.tex <==
\begin{figure}[h]
\centering
\begin{tikzpicture}[every loop/.style={}]
    % draw states
    \node[circle, draw, minimum size = 3cm,label = center:$s_{1}$] (s1) {};
    \node[circle, draw, minimum size = 3cm, right=3cm of s1, label = center:$s_{2}$] (s2) {};
    \node[inner sep=5pt, minimum size = 3cm, right = 3cm of s2, label = center:$\cdots$] (dots) {};
    \node[circle, draw, minimum size = 3cm, right=3cm of dots, label = center:$s_{N - 1}$] (spen) {};
    \node[circle, draw, minimum size = 3cm, right=3cm of spen, label = center:$s_{N}$] (sfin) {};

    % draw rewards
    \node[left = .5cm of s1] (rwd1) {$r = 0$};
    \node[right = .5cm of sfin] (rwd1) {$r = 1$};

    % draw transitions: upstream   
    \path[-{Latex[length=.5cm]}, draw, black] (sfin) edge  [loop above] node {\small$1 - \frac{1}{N}$} ();
    \draw[black, -{Latex[length=.5cm]}] (1.5, 1.25) to [bend left=45] node [above = .25cm]{\small$1 - \frac{1}{N}$} (4.5, 1.25) ;
    \draw[red, -{Latex[length=.5cm]}] (4.5, 1.05) to [bend left=45] node [below= .25cm]{\small$\frac{1}{N}$} (1.5, 1.05);

    \draw[black, -{Latex[length=.5cm]}] (7.5, 1.25) to [bend left=45] node [above = .25cm]{\small$1 - \frac{1}{N}$} (10.5, 1.25) ;
    \draw[red, -{Latex[length=.5cm]}] (10.5, 1.05) to [bend left=45] node [below= .25cm]{\small$\frac{1}{N}$} (7.5, 1.05);

    \draw[black, -{Latex[length=.5cm]}] (13.5, 1.25) to [bend left=45] node [above = .25cm]{\small$1 - \frac{1}{N}$} (16.5, 1.25) ;
    \draw[red, -{Latex[length=.5cm]}] (16.5, 1.05) to [bend left=45] node [below= .25cm]{\small$\frac{1}{N}$} (13.5, 1.05);

    \draw[black, -{Latex[length=.5cm]}] (19.5, 1.25) to [bend left=45] node [above = .25cm]{\small$1 - \frac{1}{N}$} (22.5, 1.25) ;
    \draw[red, -{Latex[length=.5cm]}] (22.5, 1.05) to [bend left=45] node [below= .25cm]{\small$\frac{1}{N}$} (19.5, 1.05);

    % \path[-{Latex[length=.5cm]}, draw, black] (sfin) edge  [loop above] node {$1 - \frac{1}{N}$} ();
    
    % draw transitions: downstream
    \path[-{Latex[length=.5cm]}, draw, blue] (s1) edge  [loop below] node {\small$1$} ();
    \draw[blue, -{Latex[length=.5cm]}] (6 - .75, -1.7) to [bend left=60] node [below = .25cm]{\small$1$} (0 + .75, -1.7);

    \draw[blue, -{Latex[length=.5cm]}] (12 - .75, -1.7) to [bend left=60] node [below = .25cm]{\small$1$} (6 + .75, -1.7);

    \draw[blue, -{Latex[length=.5cm]}] (18 - .75, -1.7) to [bend left=60] node [below = .25cm]{\small$1$} (12 + .75, -1.7);
    
    \draw[blue, -{Latex[length=.5cm]}] (24 - .75, -1.7) to [bend left=60] node [below = .25cm]{\small$1$} (18 + .75, -1.7);
\end{tikzpicture}

\caption{Chain MDP \citep{ChainMDP}: $\abs{\mathcal{S}} = H = N$.}
\end{figure}
